Jet-regulated cooling catastrophe

We present the first implementation of Active Galactic Nuclei (AGN) feedback in the form of momentum driven jets in an Adaptive Mesh Refinement (AMR) cosmological resimulation of a galaxy cluster. The jets are powered by gas accretion onto Super Massive Black Holes (SMBHs) which also grow by mergers. Throughout its formation, the cluster experiences different dynamical states: both a morphologically perturbed epoch at early times and a relaxed state at late times allowing us to study the different modes of BH growth and associated AGN jet feedback. BHs accrete gas efficiently at high redshift (z>2), significantly pre-heating proto-cluster halos. Gas-rich mergers at high redshift also fuel strong, episodic jet activity, which transports gas from the proto-cluster core to its outer regions. At later times, while the cluster relaxes, the supply of cold gas onto the BHs is reduced leading to lower jet activity. Although the cluster is still heated by this activity as sound waves propagate from the core to the virial radius, the jets inefficiently redistribute gas outwards and a small cooling flow develops, along with low-pressure cavities similar to those detected in X-ray observations. Overall, our jet implementation of AGN feedback quenches star formation quite efficiently, reducing the stellar content of the central cluster galaxy by a factor 3 compared to the no AGN case. It also dramatically alters the shape of the gas density profile, bringing it in close agreement with the beta model favoured by observations, producing quite an isothermal galaxy cluster for gigayears in the process. However, it still falls short in matching the lower than Universal baryon fractions which seem to be commonplace in observed galaxy clusters.

==> PaxHeader/article.tex <==
17 gid=784332012
18 uid=1861002210
20 ctime=1278672749
20 atime=1278673000
38 LIBARCHIVE.creationtime=1274974037
24 SCHILY.dev=234881027
21 SCHILY.ino=873271
18 SCHILY.nlink=1

